Assessing the impact of emergency department short stay units using length-of-stay prediction and discrete event simulation

Accurately predicting hospital length-of-stay at the time a patient is admitted to hospital may help guide clinical decision making and resource allocation. In this study we aim to build a decision support system that predicts hospital length-of-stay for patients admitted to general internal medicine from the emergency department. We conduct an exploratory data analysis and employ feature selection methods to identify the attributes that result in the best predictive performance. We also develop a discrete-event simulation model to assess the performances of the prediction models in a practical setting. Our results show that the recommendation performances of the proposed approaches are generally acceptable and do not benefit from the feature selection. Further, the results indicate that hospital length-of-stay could be predicted with reasonable accuracy (e.g., AUC value for classifying short and long stay patients is 0.69) using patient admission demographics, laboratory test results, diagnostic imaging, vital signs and clinical documentation.

==> tables/MLRess/confusion.tex <==
\begin{tabular}{lcccc}
\toprule
& TP    & TN    &  FP   & FN \\
\midrule
LDA - Count     & 354   & 937   & 165   & 726 \\
XGB - Count     & 721   & 700   & 402   & 359 \\
\midrule
XGB - Actual Mean LOS (hr)  & 323   & 45    & 46    & 227 \\
XGB - Actual Median LOS (hr)& 190   & 44    & 46    & 155 \\
XGB - Actual LOS $\sigma$ (hr)& 417 & 17    & 18    & 275 \\
\midrule
\end{tabular}

==> tables/MLRess/tbr_LDA.tex <==
\newcommand{\mcp}{\multicolumn{1}{p{1.95cm}}}
\newcommand{\mcps}{\multicolumn{1}{p{1.3cm}}}
\newcommand{\mro}{\multirow{2}{3.6cm}}
\newcommand{\mrt}{\multirow{2}{0.7cm}}
\newcommand{\cnt}{\centering}
\newcommand{\rrt}{\raggedright}
\begin{footnotesize}
\scalebox{0.85}{
\begin{tabular}{lccccccc}
\toprule
\mro{\rrt Feature Selection Method} & \mcps{\cnt CV\\ Accuracy} & \mcps{\cnt CV\\ Variance} & \mcps{\cnt Accuracy\\} & \mcps{\cnt Precision\\ (LS)} & \mcps{\cnt Precision\\ (SS)} & \mcps{\cnt Recall\\ (LS)} & \mcps{\cnt Recall\\ (SS)} \\
\midrule
Without feature selection & 0.615 & 0.013 & 0.617 & 0.616 & 0.618 & 0.619 & 0.615 \\ 
Ensemble & 0.611 & 0.019 & 0.608 & 0.646 & 0.586 & 0.476 & 0.740 \\ 
%Mutual information (regression) & 0.585 & 0.007 & 0.597 & 0.601 & 0.593 & 0.573 & 0.620 \\ 
%F-statistic (regression) & 0.585 & 0.012 & 0.612 & 0.605 & 0.622 & 0.647 & 0.578 \\ 
Chi-squared & 0.580 & 0.011 & 0.582 & 0.590 & 0.574 & 0.529 & 0.634 \\ 
%F-statistic (classification) & 0.569 & 0.005 & 0.564 & 0.573 & 0.557 & 0.500 & 0.628 \\
F-statistic & 0.569 & 0.005 & 0.564 & 0.573 & 0.557 & 0.500 & 0.628 \\ 
%Mutual information (classification) & 0.560 & 0.008 & 0.548 & 0.547 & 0.548 & 0.546 & 0.550 \\
Mutual information & 0.560 & 0.008 & 0.548 & 0.547 & 0.548 & 0.546 & 0.550 \\ 
Pearson & 0.537 & 0.051 & 0.501 & 0.000 & 0.501 & 0.000 & 1.000 \\ 
Spearman & 0.546 & 0.002 & 0.555 & 0.555 & 0.555 & 0.548 & 0.562 \\ 
\bottomrule
\end{tabular}
}
\end{footnotesize}

==> tables/MLRess/tbr_LR.tex <==
\begin{tabular}{p{5cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}}
    \toprule
    Feature Selection Method & CV Accuracy & CV Variance & Accuracy & Precision (long stay) & Precision (short stay) & Recall (long stay) & Recall (short stay) \\
        \midrule
Without feature selection & 0.512 & 0.009 & 0.525 & 0.538 & 0.519 & 0.353 & 0.698 \\ 
Pearson & 0.618 & 0.012 & 0.618 & 0.618 & 0.619 & 0.618 & 0.618 \\ 
Chi-squared & 0.577 & 0.013 & 0.580 & 0.587 & 0.573 & 0.531 & 0.628 \\ 
Mutual information (classification) & 0.560 & 0.008 & 0.548 & 0.547 & 0.548 & 0.546 & 0.550 \\ 
Spearman & 0.546 & 0.002 & 0.555 & 0.555 & 0.555 & 0.548 & 0.561 \\ 
F-statistic (classification) & 0.545 & 0.005 & 0.552 & 0.551 & 0.552 & 0.550 & 0.553 \\ 
Ensemble & 0.508 & 0.010 & 0.522 & 0.520 & 0.524 & 0.545 & 0.500 \\ 
Mutual information (regression) & 0.508 & 0.010 & 0.520 & 0.518 & 0.522 & 0.547 & 0.494 \\ 
F-statistic (regression) & 0.502 & 0.003 & 0.514 & 0.523 & 0.511 & 0.313 & 0.715 \\ 

        \bottomrule
    \end{tabular}

==> tables/MLRess/tbr_NB.tex <==
\begin{tabular}{p{5cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}}
    \toprule
    Feature Selection Method & CV Accuracy & CV Variance & Accuracy & Precision (long stay) & Precision (short stay) & Recall (long stay) & Recall (short stay) \\
        \midrule
Without feature selection & 0.545 & 0.005 & 0.560 & 0.607 & 0.542 & 0.338 & 0.782 \\ 
Pearson & 0.593 & 0.008 & 0.597 & 0.638 & 0.575 & 0.445 & 0.749 \\ 
Chi-squared & 0.566 & 0.009 & 0.554 & 0.569 & 0.545 & 0.440 & 0.668 \\ 
Mutual information (classification) & 0.566 & 0.007 & 0.559 & 0.582 & 0.546 & 0.411 & 0.706 \\ 
F-statistic (classification) & 0.546 & 0.006 & 0.550 & 0.593 & 0.534 & 0.312 & 0.786 \\ 
Spearman & 0.543 & 0.008 & 0.560 & 0.590 & 0.545 & 0.387 & 0.732 \\ 
Ensemble & 0.521 & 0.009 & 0.518 & 0.522 & 0.515 & 0.408 & 0.627 \\ 
Mutual information (regression) & 0.521 & 0.009 & 0.517 & 0.521 & 0.515 & 0.409 & 0.625 \\ 
F-statistic (regression) & 0.517 & 0.010 & 0.521 & 0.523 & 0.519 & 0.458 & 0.584 \\ 

        \bottomrule
    \end{tabular}

==> tables/MLRess/tbr_RF.tex <==
\begin{tabular}{p{5cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{1.3cm}}
    \toprule
    Feature Selection Method & CV Accuracy & CV Variance & Accuracy & Precision (long stay) & Precision (short stay) & Recall (long stay) & Recall (short stay) \\
        \midrule
Without feature selection & 0.573 & 0.011 & 0.579 & 0.600 & 0.566 & 0.470 & 0.688 \\ 
Pearson & 0.575 & 0.001 & 0.561 & 0.571 & 0.554 & 0.489 & 0.633 \\ 
Ensemble & 0.575 & 0.011 & 0.580 & 0.597 & 0.567 & 0.484 & 0.674 \\ 
F-statistic (classification) & 0.556 & 0.009 & 0.561 & 0.578 & 0.550 & 0.446 & 0.675 \\ 
Mutual information (regression) & 0.553 & 0.004 & 0.560 & 0.574 & 0.550 & 0.458 & 0.661 \\ 
Mutual information (classification) & 0.548 & 0.008 & 0.563 & 0.571 & 0.556 & 0.496 & 0.629 \\ 
F-statistic (regression) & 0.547 & 0.007 & 0.553 & 0.564 & 0.545 & 0.460 & 0.645 \\ 
Chi-squared & 0.537 & 0.004 & 0.558 & 0.575 & 0.548 & 0.444 & 0.672 \\ 
Spearman & 0.515 & 0.009 & 0.521 & 0.521 & 0.522 & 0.516 & 0.527 \\ 

        \bottomrule
    \end{tabular}

==> tables/MLRess/tbr_XGB.tex <==
\newcommand{\mcp}{\multicolumn{1}{p{1.95cm}}}
\newcommand{\mcps}{\multicolumn{1}{p{1.3cm}}}
\newcommand{\mro}{\multirow{2}{3.6cm}}
\newcommand{\mrt}{\multirow{2}{0.7cm}}
\newcommand{\cnt}{\centering}
\newcommand{\rrt}{\raggedright}
\begin{footnotesize}
\scalebox{0.85}{
\begin{tabular}{lccccccc}
\toprule
\mro{\rrt Feature Selection Method} & \mcps{\cnt CV\\ Accuracy} & \mcps{\cnt CV\\ Variance} & \mcps{\cnt Accuracy\\} & \mcps{\cnt Precision\\ (LS)} & \mcps{\cnt Precision\\ (SS)} & \mcps{\cnt Recall\\ (LS)} & \mcps{\cnt Recall\\ (SS)} \\
\midrule
Without feature selection & 0.629 & 0.011 & 0.646 & 0.646 & 0.647 & 0.645 & 0.647 \\ 
Ensemble & 0.631 & 0.008 & 0.634 & 0.629 & 0.639 & 0.650 & 0.617 \\ 
%Mutual information (regression) & 0.599 & 0.006 & 0.614 & 0.616 & 0.612 & 0.604 & 0.624 \\ 
%Mutual information (classification) & 0.586 & 0.006 & 0.598 & 0.598 & 0.599 & 0.599 & 0.598 \\ 
%F-statistic (regression) & 0.586 & 0.008 & 0.599 & 0.588 & 0.613 & 0.658 & 0.541 \\ 
Chi-squared & 0.570 & 0.011 & 0.585 & 0.593 & 0.579 & 0.542 & 0.629 \\ 
%F-statistic (classification) & 0.569 & 0.008 & 0.586 & 0.599 & 0.576 & 0.516 & 0.655 \\
F-statistic & 0.569 & 0.008 & 0.586 & 0.599 & 0.576 & 0.516 & 0.655 \\
Mutual information & 0.586 & 0.006 & 0.598 & 0.598 & 0.599 & 0.599 & 0.598 \\ 
Pearson & 0.611 & 0.012 & 0.621 & 0.617 & 0.625 & 0.635 & 0.607 \\ 
Spearman & 0.547 & 0.002 & 0.563 & 0.568 & 0.559 & 0.525 & 0.601 \\ 
\bottomrule
\end{tabular}
}
\end{footnotesize}

==> tables/others/des_results_GW_CAPACITY_70_small.tex <==

%\resizebox{\textwidth}{!}{%

\begin{tabular}{lrrrr}
        \toprule& perfect & random & RF & XGB \\
        \midrule
Total sterilization count & 7,332 & 8,077 & 7,929 & 8,059 \\
SSU sterilization count & 1,515 & 1,907 & 1,911 & 1,962 \\
GW sterilization count & 3,584 & 4,007 & 3,905 & 3,893 \\
Waiting area sterilization count & 2,233 & 2,163 & 2,113 & 2,204 \\
Average GW wait time (hr) & 13.5 & 7.9 & 8.5 & 7.5 \\
average LS time in SSU (hr) & 0.0 & 53.2 & 53.5 & 53.5 \\
average LS time in GW (hr) & 234.6 & 224.4 & 225.6 & 225.3 \\
average SS time in SSU (hr) & 39.7 & 36.3 & 36.9 & 35.7 \\
average SS time in GW (hr) & 13.3 & 31.6 & 30.2 & 31.5 \\
\# LS misclassifications & 0 & 1,537 & 1,261 & 1,401 \\
\# SS misclassifications & 0 & 777 & 542 & 495\\
\bottomrule
        \end{tabular}
        %}


==> tables/others/des_results_GW_CAPACITY_70_small_new.tex <==

%\resizebox{\textwidth}{!}{%

\begin{tabular}{lrrrr}
        \toprule& perfect & random & RF & XGB \\
        \midrule
        Total sterilization count & 6575& 6820& 6666& 6645\\
SSU sterilization count & 3535& 3073& 3213& 3144\\
GW sterilization count & 3040& 3747& 3453& 3501\\
Average GW wait time (hr) & 12.23& 3.63& 2.14& 5.87\\
average LS time in SSU (hr) & 12.23& 27.55& 29.54& 22.47\\
average LS time in GW (hr) & 156.11& 140.79& 138.80& 145.87\\
average SS time in SSU (hr) & 14.99& 8.76& 10.84& 10.59\\
average SS time in GW (hr) & 0.00& 6.24& 4.15& 4.40\\
\# LS misclassifications & 0& 1577& 1751& 1110\\
\# SS misclassifications & 0& 767& 458& 536\\
\bottomrule
        \end{tabular}
        %}


==> tables/others/des_results_GW_CAPACITY_inf_small.tex <==

%\resizebox{\textwidth}{!}{%

\begin{tabular}{lrrrr}
        \toprule& perfect & random & RF & XGB \\
        \midrule
Total sterilization count & 5,207 & 6,440 & 6,224 & 6,388 \\
SSU sterilization count & 1,557 & 2,313 & 2,276 & 2,463 \\
GW sterilization count & 3,650 & 4,127 & 3,948 & 3,925 \\
Waiting area sterilization count & 0 & 0 & 0 & 0 \\
Average GW wait time (hr) & 0 & 0 & 0 & 0 \\
average LS time in SSU (hr) & 0.0 & 72.0 & 72.0 & 72.0 \\
average LS time in GW (hr) & 254.5 & 229.7 & 234.2 & 232.0 \\
average SS time in SSU (hr) & 38.9 & 38.4 & 38.2 & 38.3 \\
average SS time in GW (hr) & 0.0 & 36.1 & 33.2 & 32.0 \\
\# LS misclassifications & 0 & 1,538 & 1,261 & 1,401 \\
\# SS misclassifications & 0 & 782 & 542 & 495\\
\bottomrule
        \end{tabular}
        %}


==> tables/others/selected_columns.tex <==
\resizebox{\textwidth}{!}{\begin{tabular}{ll}
\toprule
\textbf{Column name} & \textbf{Selected by method} \\
\midrule
NON\_GIM\_ER.CONSULT & spearman (p:0.0, s:0.02)\\
admit\_timestamp & f\_regression (p:0.0, s:4633.3),mutual\_info\_regression (p:nan, s:0.07)\\
admit\_via\_ambulance & spearman (p:0.0, s:0.1),f\_classif (p:0.0, s:169.33),mutual\_info\_classif (p:nan, s:0.0)\\
age & pearson (p:0.0, s:0.09),f\_regression (p:0.0, s:4896.92),mutual\_info\_regression (p:nan, s:0.02)\\
current\_visit\_bad\_lab\_result\_with\_percentile\_75\_ratio & chi2 (p:0.0, s:201.18)\\
current\_visit\_lab\_test\_count & chi2 (p:0.0, s:465.83)\\
current\_visit\_lab\_uniq\_test\_count & chi2 (p:0.0, s:323.95)\\
er\_diag\_code & mutual\_info\_classif (p:nan, s:0.07),chi2 (p:0.0, s:326.88)\\
gender & spearman (p:0.02, s:0.02),chi2 (p:0.0, s:817.2)\\
lab\_ABASO & chi2 (p:0.0, s:407.05)\\
lab\_ADDON & chi2 (p:0.0, s:163.44)\\
lab\_AEOS & chi2 (p:0.0, s:316.29)\\
lab\_AGAP & chi2 (p:0.0, s:370.63)\\
lab\_ALB & pearson (p:0.0, s:0.16),mutual\_info\_regression (p:nan, s:0.04),chi2 (p:0.0, s:1149.78)\\
lab\_ALYMP & pearson (p:0.0, s:0.08)\\
lab\_BLC & f\_classif (p:0.0, s:139.26)\\
lab\_GLOB & pearson (p:0.0, s:0.1)\\
lab\_HGB & pearson (p:0.0, s:0.08)\\
lab\_LIMIT & f\_classif (p:0.0, s:154.2),mutual\_info\_classif (p:nan, s:0.0)\\
lab\_LYMP & pearson (p:0.0, s:0.09)\\
lab\_RBC & pearson (p:0.0, s:0.08)\\
lab\_RDW & mutual\_info\_regression (p:nan, s:0.02)\\
lab\_RINR & pearson (p:0.0, s:0.08)\\
lab\_RPT & pearson (p:0.0, s:0.08)\\
lab\_UAPR & spearman (p:0.0, s:0.08),f\_classif (p:0.0, s:176.81),mutual\_info\_classif (p:nan, s:0.01)\\
lab\_UBIL & f\_classif (p:0.0, s:148.49)\\
lab\_UBLD & f\_classif (p:0.0, s:150.16),mutual\_info\_classif (p:nan, s:0.0)\\
lab\_UCOL & f\_classif (p:0.0, s:150.16),mutual\_info\_classif (p:nan, s:0.0)\\
lab\_UKETO & f\_classif (p:0.0, s:149.6)\\
lab\_UNIT & f\_classif (p:0.0, s:150.16),mutual\_info\_classif (p:nan, s:0.0)\\
lab\_UPRO & spearman (p:0.0, s:0.05),mutual\_info\_classif (p:nan, s:0.01)\\
lab\_URBC & mutual\_info\_classif (p:nan, s:0.01)\\
lab\_UREA & pearson (p:0.0, s:0.1),mutual\_info\_regression (p:nan, s:0.02)\\
lab\_UWBC & f\_classif (p:0.0, s:114.96),mutual\_info\_classif (p:nan, s:0.01)\\
ordered\_datetime & mutual\_info\_regression (p:nan, s:0.04)\\
previous\_encounter\_los\_mins\_max & f\_regression (p:0.0, s:4614.28)\\
previous\_encounter\_most\_recent\_los & f\_regression (p:0.0, s:4614.28)\\
previous\_ip\_diag\_count & f\_regression (p:0.0, s:4614.28)\\
previous\_ip\_diag\_mode & f\_regression (p:0.0, s:4614.28)\\
previous\_lab\_test\_count & f\_regression (p:0.0, s:4614.28)\\
previous\_lab\_test\_uniq\_count & f\_regression (p:0.0, s:4614.28)\\
\midrule
readmission & f\_regression (p:0.0, s:4784.87)\\
triage\_dayofweek & mutual\_info\_regression (p:nan, s:0.09)\\
triage\_time\_of\_day & mutual\_info\_regression (p:nan, s:0.21)\\
triage\_timestamp & f\_regression (p:0.0, s:4633.3),mutual\_info\_regression (p:nan, s:0.06)\\
vit\_Oxygen Flow Rate (L/Min) & spearman (p:0.0, s:0.04)\\
vit\_current\_visit\_vital\_test\_count & mutual\_info\_regression (p:nan, s:0.02)\\
\bottomrule
    \end{tabular}}
